Cross-Domain First Person Audio-Visual Action Recognition through Relative Norm Alignment

First person action recognition is an increasingly researched topic because of the growing popularity of wearable cameras. This is bringing to light cross-domain issues that are yet to be addressed in this context. Indeed, the information extracted from learned representations suffers from an intrinsic environmental bias. This strongly affects the ability to generalize to unseen scenarios, limiting the application of current methods in real settings where trimmed labeled data are not available during training. In this work, we propose to leverage over the intrinsic complementary nature of audio-visual signals to learn a representation that works well on data seen during training, while being able to generalize across different domains. To this end, we introduce an audio-visual loss that aligns the contributions from the two modalities by acting on the magnitude of their feature norm representations. This new loss, plugged into a minimal multi-modal action recognition architecture, leads to strong results in cross-domain first person action recognition, as demonstrated by extensive experiments on the popular EPIC-Kitchens dataset.

==> latex/Tables/Ablation2.tex <==
% \usepackage{multirow}


\begin{table}
\centering


\begin{tabular}{l|lr}
\multicolumn{2}{l}{Ablations}                     & \multicolumn{1}{l}{Mean}  \\ \hline \hline
\multirow{4}{*}{Baseline} & Supervised Target & 59,76                     \\
                             & Source Only       & 40,93               \\
                             & Deep All          & 44,67                    \\ \hline
\multirow{4}{*}{HNA}         & Supervised Target & 62,41               \\
                             & DG                & 44,58               \\
                             & Multi DG          & 46,7     \\ 
                             & DA                & 47,19             \\ \hline
\multirow{4}{*}{RNA}         & Supervised Target & 63,13               \\
                             & DG                & 45,75                   \\
                             & Multi DG          & 51,06               \\ 
                             & DA                & 47,71      \\ \hline
\multirow{4}{*}{Fusion}      & Supervised Target & 60,18                     \\ 
                             & Source Only       & 40,33               \\
                             & Deep All          & 47,61      
                                         \\ \hline
\multirow{4}{*}{RNA - Fusion}  & Supervised Target & 62,11               \\
                             & DG                & 45,48               \\
                             & Multi DG          & 49,56      \\ 
                             & DA                & 45,73                  \\  \hline
\end{tabular}
\end{table}

==> latex/Tables/multi-modal-da.tex <==
\begin{table*}[thb!]
\centering
\begin{adjustbox}{width=0.7\columnwidth, margin=0ex 1ex 0ex 0ex}
\begin{tabular}{l|cccccc|c}
\hline \hline
Multi-Modal                & \multicolumn{1}{c}{D1 $\rightarrow$ D2} & D1 $\rightarrow$ D3 & D2  $\rightarrow$ D1 & D2 $\rightarrow$ D3 & D3  $\rightarrow$ D1 & D3  $\rightarrow$ D2    & Mean \\ \hline \hline
SS Only         &       44,83                   &  42,88     &   40,61   &   54,21   &   42,58    &    53,5 & 46,44  \\ %\hline
Adversarial Only         &          41,02                  &   43,04     &  39,36     &  49,25      & 38,77      &     50,56     &      43,67     \\ %\hline
MMSADA \cite{Munro_2020_CVPR}         &         48,9                   &  46,66    &  39,51    &   50,89    & 45,42      &55,14 & 47,75        \\ %\hline
MMD \cite{da-mmdlong2015learning}         &        42,4                   &  43,84     &  40,87    &  48,13   & 41,46        &50,03  & 44,46        \\ %\hline
AdaBN \cite{ada-bn}         &       36,64                   &  42,57    & 33,97      &   46,63    & 40,51        &  51,2 & 41,92        \\ \hline

RNA  (Ours)      &       46,89                  &  48,4   &   41,58   &  51,77    &   43,19    &    54,43 & 47,71  \\ %\hline
RNA + GRL (Ours)      &       \underline{47,54}                 &  47,71   &  43,19   &  52,83    &   43,02    &    54,1 & \textbf{48,07 } \\ \hline


\end{tabular}
\end{adjustbox}
\caption{}
\label{tab:multi-modal-da}

\end{table*}


==> latex/Tables/multi-source-dg.tex <==
\begin{table}[t]
\begin{adjustbox}{width=1.0\columnwidth, margin=0ex 1ex 0ex 0ex}
\begin{tabular}{lccccccc}
\hline \hline
Multi-Source  & \multicolumn{1}{c}{D1, D2  $\rightarrow$ D3} & D1, D3  $\rightarrow$ D2 & D2, D3  $\rightarrow$ D1 & Mean\\ \hline
Deep All      &       51,47                    &   43,19   & 39,35 & 44,67 \\ \hline
AlignLoss       &       50,01                   &   42,4   & 44,4 & 45,6 \\ \hline
OrthLoss     &       53,08                  &    41,76  &  48,07 &  47,64\\ \hline
Norm     &       52,07                    &   42,63  &  45,14 &  46,61 \\ \hline
SS            &       51,87                     &  39,79   & 52,73 & 48,13    \\ \hline
RNA (Ours) &      55,88                     &   45,65    &   51,64 &  \textbf{51,06} \\ \hline 
\hline
\end{tabular}
\end{adjustbox}
\caption{}
\label{tab:multi-source-dg}

\end{table}


==> latex/Tables/single-modality.tex <==
\begin{table*}[hbt!]
\begin{tabular}{lccccccc}
\hline \hline
           & \multicolumn{1}{c}{D1 $\rightarrow$ D2} & D1 $\rightarrow$ D3 & D2 $\rightarrow$ D1     & D2 $\rightarrow$ D3     & D3 $\rightarrow$ D1     & D3 $\rightarrow$ D2   & Mean  \\ \hline
Source Only (RGB) &      34,15                      &    35,03  &     34,76    &  38,79       &      33,03    &    41,08     &  36,14  \\ \hline
Source Only (Audio) &     31,90                      &   36,49    &   29,17       &   44,00       &     34,00    &  42,93 & 36,42        \\ \hline
Source Only (RGB+Audio) &    39,03&	39,17	&35,27&	47,52&	40,26&	49,98&	41,87       \\ \hline
\hline
Supervised (RGB) & \multicolumn{2}{c}{51,72}              & \multicolumn{2}{c}{61,65} & \multicolumn{2}{c}{60,37} & 57,91 \\ \hline 

Supervised (Audio) & \multicolumn{2}{c}{45,24}              & \multicolumn{2}{c}{58,83} & \multicolumn{2}{c}{61,56} & 55,21\\ \hline 

Supervised (RGB+Audio)  & \multicolumn{2}{c}{50,30}              & \multicolumn{2}{c}{64,40} & \multicolumn{2}{c}{63,50} & \textbf{59,40}\\ \hline \hline
\end{tabular}
\caption{Top-1 accuracy of (nome dell'esperimento. Single modality non so se e' corretto visto che abbiamo anche il multi). Source Only: train on source $\mathcal{S}$ and test on target $\mathcal{T}$ ($\mathcal{S}$ $\rightarrow$ $\mathcal{T}$). Supervised: train and test on $\mathcal{T}$ ($\mathcal{T}$ $\rightarrow$ $\mathcal{T}$)}
\label{tab:single-mod}

\end{table*}

==> latex/Tables/single-source-dg.tex <==
\begin{table}[t]
\begin{adjustbox}{width=1.0\columnwidth, margin=0ex 1ex 0ex 0ex}
\begin{tabular}{l|cccccc|c}
% OPPURE
%\begin{tabularx}{\columnwidth}{X|XXXXXXX}

\hline

             & \multicolumn{1}{c}{D1 $\rightarrow$ D2} & D1 $\rightarrow$ D3 & D2  $\rightarrow$ D1     & D2 $\rightarrow$  D3     & D3  $\rightarrow$ D1     & D3  $\rightarrow$ D2   & Mean   \\ \hline
Source Only &    39,03&	39,17	&35,27&	47,52&	40,26&	49,98&	41,87  \\ \hline \hline
AlignLoss   &    38,50                        &   33,75    &     32,59       &    45,78       &    39,97       &      50,86 & 41,76     \\ \hline
OrthLoss     &    39,18                        &    37,55    &      36,86      &     47,09      &      43,70    &       51,61   & 42,67 \\ \hline
Norm    &   40,03                        &    39,88    &      36,39      &    48,47     &     42,60     &      48,33    & 42,62 \\ \hline
SS   &    38,86                        &    33,75   &      32,59      &     45,78     &       39,97     &       50,86    & 40,30 \\ \hline

RNA (Ours) &      45,01                      &  44,62   &    41,76     &    48,90       &       42,20  &    51,98 & \textbf{45,75}       \\ \hline

\hline

%\end{tabularx}

\end{tabular}
\end{adjustbox}

\caption{Top-1 accuracy of multi-modal single-source domain generalization setting.}
\label{tab:single-source-dg}
\end{table}

==> latex/Tables/tbn-fusion.tex <==
\begin{table*}[hbt!]
\begin{tabular}{lcccccc}
\hline
\hline
Fusion             & \multicolumn{1}{c}{D1 $\rightarrow$ D2} & D1 $\rightarrow$ D3 & D2  $\rightarrow$ D1     & D2  $\rightarrow$  D3     & D3  $\rightarrow$ D1     & D3  $\rightarrow$ D2     \\ \hline

\hline
TBN (Source Only) &                           &       &           &           &           &           \\ \hline
TBN (DG) &                            &       &           &           &           &           \\ \hline
TBN (DA) &                            &       &           &           &           &           \\ \hline
TBN Supervised &                            &       &           &           &           &           \\ \hline \hline
Ours RELATIVE Fusion (Source Only) &     \checkmark                       &    \checkmark   &     \checkmark      &    \checkmark       &      \checkmark     &      \checkmark     \\ \hline
Ours RELATIVE Fusion (DG) &     \checkmark                       &     \checkmark  &    \checkmark       &    \checkmark       &       \checkmark    &     \checkmark      \\ \hline

Ours RELATIVE + GRL Fusion (DA) &                       \checkmark   &  \checkmark     &     \checkmark      &   \checkmark        &   \checkmark        &     \checkmark      \\ \hline

Supervised Fusion   & \multicolumn{2}{c}{\checkmark}              & \multicolumn{2}{c}{\checkmark} & \multicolumn{2}{c}{\checkmark} \\ \hline \hline
\end{tabular}
\caption{}

\end{table*}
